Towards Controlling Refinements of Statecharts

In incremental development strategies, modelers frequently refine Statecharts models to satisfy requirements and changes. Although several solutions exist to the problem of Statecharts refinement, they provide such levels of freedom that a statechart cannot make assumptions or guarantees about its future structure. In this paper, we propose a set of bounding rules to limit the allowable Statecharts refinement operations such that certain assumptions will hold.

==> implementation.tex <==

\section{Implementation} \label{sec:implementation}

We now describe how Statechart refinement is performed using our implementation in \ATOM{}~\cite{Mannadiar2012}.

\subsection{Process}

\begin{figure}[ht]
	\centering
	\epsfig{file=images/classdiagram.eps, width=\linewidth}
	\caption{The class diagram for the refiner and validator}
	\label{fig:cd}
\end{figure}
%
\vspace{-0.50\baselineskip}
The designer of a particular statechart first constructs the statechart within \ATOM{}.
Once this design is complete and well-formed, the refinement process should begin.
The developer initiates the ``refine'' command within the tool, which changes \ATOM{} from \emph{Edit} mode to \emph{Refine} mode. 
This mode limits certain user activities, such as deleting original elements, adding additional elements outside of a \Virtual{} region, etc.
An additional result of switching modes is that the original model is replicated to a new window in which the developer will perform refinements, such that the original model is not being modified during the refinement process.
The developer then selects which elements he would like to refine, issues the ``refine'' command, and then a wizard pops up to walk the user through the refinement process. 
The refiner implementation automatically generates a mapping between every refined or created element and an original element.
This can result in many mappings to a single original source element.
When the developer is satisfied with the refined statechart, he initiates the ``validate'' command in order to validate the model, though invalid models are allowed to be saved.
This is to prevent blocking the developer from introducing technically invalid structures that will only be invalid temporarily.
The validator then checks the refined elements against the rules defined within \Sect{sec:refine}.

%In our implementation, we utilize the tool \ATOM{}, which is a modeling tool being developed as an international effort by multiple Universities. 
%The designer of a particular statechart first constructs the statechart within \ATOM{}. 
%Once this design is found to be sound (various testing, inspection, etc), and the base model is deemed to be stable, the developer initiates the ``refine'' command within the tool, which modifies the filename to ``ORIGINALNAME\_r\#'' where ``r\#'' indicates the current refinement level. 
%This command changes the tool from ``Edit'' mode to ``Refine'' mode, where certain user behaviors are outright prevented, such as the deletion of original elements, the addition of elements outside of \Virtual{} regions, and the renaming of original elements. 
%Any elements that are created through refinement can be modified freely, within bounds of the constraints of the refinement rules. 
%The current implementation requires an explicit call to \Model{Validator}, either during a save operation or at the developers discretion, which was a decision made in order to prevent blocking the designer for errors that may exist only temporarily. 
%The developer then selects an element to refine, issues the ``refine'' command, and is then presented with a dialog of available refinement operations for the given selection. 
%If multiple elements are selected, then multiple dialog boxes will prompt the user in order to determine the refinement operations for each element. The developer selects which refinement to apply (such as Basic -> OR, Transition -> Split [transition-state-transition], Transition -> Fork [splits the current transition into two transitions side by side], etc). The appropriate refiner is then called, the contents from the original element are cloned into the newly created refined element, and then the original is replaced by the refined element on the canvas.


\subsection{Design}

\Fig{fig:cd} illustrates an excerpt of the overall design of our implementation.
The \Code{\ATOM{}} singleton holds triggers for both the refine and validate commands. 
Each of these forwards on the request to the respective \Code{Validator} or \Code{Refiner} singletons, which handle type processing and user prompting where needed.
\Code{Refiner} contains one instance of each subclass of \Code{BaseRefiner}. 
The \Code{BaseRefiner} class and its subclasses follow the Template pattern.
The refiners present within this design are meant to create a convenience method for creating the mappings from an original statechart to a refined statechart, though mappings could conceivably be made manually between two statecharts and the \Code{MappingValidator} will still determine whether or not the mappings are correct.
The validator contains both a \Code{MappingValidator} and an \Code{SCValidator} object.
The \Code{MappingValidator} iterates through all of the mappings and evaluates all of the applied constraints until the list is either exhausted or a \Code{FAIL} result is returned.
The \Code{SCValidator} class validates that the current statechart is fully defined (\ie{} no abstract elements remain) and that all originally defined elements can be mapped in the refined statechart.
We do not need to validate the refined statechart for well-formedness which is already taken care of by \ATOM{}.
The \Code{Constraint} class is a tuple of an id and a blob of data.
The \Code{evaluate} operation verifies that the mapping satisfies the specific constraint it encodes.
This class follows the Command pattern and is meant to allow easy addition of new, fully functional, self-contained constraints.
The \Code{Constraint} implementations return a \Code{ConstraintResult} as a result of their evaluation, acknowledging the satisfaction of the constraint.
We allow for \Code{NONE} and \Code{WARN} results in order to cover cases where either a constraint does not apply to the elements that it is being tested against or where mixed results (\ie{} not a complete failure or unknown) need to be returned.

\vspace*{-.75\baselineskip}%
\subsubsection{Refiner}

Algorithm~\ref{alg:baseRefiner} depicts the general behavior of the \Code{refine} operation.
The user is first prompted to specify the type of refinement to be performed on the selected element through a wizard.
For example, for the \Code{BasicRefiner}, the user must choose whether a basic state shall be refined into a basic, an OR-state, or AND-state.
The contents of the original element are then copied to the target element, such as entry/exit actions or substates.
Finally, a set of constraints applicable to this specific refined element is created along with the mappings.
%
\begin{algorithm}[H]
  \caption{The operation \Code{BaseRefiner.refine(element: SCElement)}}
  \label{alg:baseRefiner}
  \begin{algorithmic}
    {\small
    \STATE $\Code{target} \leftarrow \Code{promptRefinement(element.getType())}$
    \STATE \Code{contents} $\leftarrow$ \Code{copyContents(element)}
    \STATE \Code{applyContents(element, target)}
    \STATE \Code{generateConstraints(target)}
    \RETURN \Code{target}
    }
  \end{algorithmic}
\end{algorithm}

\vspace*{-2\baselineskip}%
\subsubsection{Validator}

Since the user still has the freedom to modify the statechart after the refiner's operations, the validator will ensure that the resulting statechart is a valid refinement with respect to the definitions given in \Sect{sec:rationale}.
In our implementation, we have realized each distinct rule from \Sect{sec:refine} as a \Code{Constraint} class.
We briefly summarize the \Code{evaluate} operation of each of these classes in what follows:
%\vspace{-\baselineskip}%
\begin{itemize}
  \item \Model{ExclusiveGuardsConstraint}: searches through all resulting transitions within a refinement mapping. If any transitions are found that are guarded, it verifies that a negation of that guard exists on another transition from the same source state. All guard validations are currently done at a literal level and do not yet allow for logically equivalent statements to be identified. This validates rule R2.4.
  %validates that any guards that exist on transitions that are refined from another transition have a mutually exclusive or default alternate path. This does not check the initial or final transitions.
  
  \item \Model{HistoryConstraint}: checks to verify that the refined history state is consistent with the rules in R7. 
  %validates that any shallow history state maps to a shallow or deep history state and that any deep history state maps only to another deep history state.
  
  \item \Model{MinimalGuardConstraint}: searches for refined transitions that are connected to the original element's source transition within a refinement mapping. For any element that is found, that element is verified to have a guard that is at least equal to the original guard allowing for some additional predicate. As with the other guard constraint, this is done at a literal string level and does not allow for alternate though equivalent logic to be used. This validates the rule defined in R2.2.
  %validates that any guard on an original transition is at least retained on the refined transition, though additional predicates are allowed. The current version does not check logical equivalence.
  
  \item \Model{OriginalBroadcastConstraint}: searches through resulting transitions within in a refinement mapping. If a transition is found to be connected to the original transition's target state, then that transition is checked to verify the presence of the original transitions broadcast event. This validates the rule defined in R2.3.
  %validates that any broadcast event on an original transition is retained on the final flow into the original target state.
  
  \item \Model{OriginalEventsConstraint}: searches through the refined transitions in a refinement mapping for the transitions connected to the original transition's source state. If such a transition is found, then the event trigger for the refined transition is validated against the original transition's event trigger. This validates the rule defined in R2.1.
  %validates that any event trigger on an original transition is retained on the initial flow out of the original source state.
  
  \item \Model{OriginalNameConstraint}: searches through the named \Code{SCElement}s within a refinement mapping for any element that matches the original element's name. This validates the requirements for named elements as defined in R1.
  %validates that the original name of a refined element is retained.
  
  \item \Model{OriginalTransitionsConstraint}:searches through states within a refinement mapping validating each state's input and output transitions against the original state's input and output transitions. This validates the original transition preservation rule defined in R1.
  %validates that any incoming and outgoing transitions on a state can still be mapped as input or output to/from that state.
  
  \item \Model{ReachabilityConstraint}: given a set refinement mapping, validates that the original transition's source and target states are reachable by performing a depth first search from the source for the target state. This validates the transition flow rule defined in R2.4.
  %validates that the original target state of a refined transition is still reachable from the original source state.
  
  \item \Model{SubstateMappingsConstraint}: searches through all of the states within a refinement mapping where the original \Code{SCElement} is a composite state.
  For every original substate, we validate that there exists a mapping to a refined substate.
  This validates the substate mapping preservation rule defined for composite states in R3 and R4.
  %validates that all original children of either an AND- or OR-state can still be mapped to the refined statechart.
\end{itemize}


==> validation.tex <==
\section{Validation} \label{sec:validation}

We are interested in applying sequences of refinements to an initial statechart, in order to reach a final design.
It is thus of the utmost importance to be able to show that sequences of refinements respect the formal refinement relation we have presented in Definition~\ref{def:refinement}.
The seven local refinement rules presented in \Sect{sec:refine} can be applied in isolation in no specific order.
In the following, we consider the flattened version of Statecharts.
Also, we focus only on rules R1 and R2 since all other Statecharts constructs considered in the remaining rules can be reduced to states and transitions through flattening.
Note that the refinement rules R1 and R2 were designed to satisfy all refinement conditions by construction.

\begin{defn}[Local Rule Application]\label{def:localRule}
  We denote by $R_s^l(SC_o) = SC_r^l$ the local application of rule R1 on a state $s \in S_o$ , where $SC_r^l$ consists of solely the newly created states and transitions, and their immediate neighbors, \ie
  $S_r^l = \bigcup_{\forall (s,s_{r_i}) \in R_s^l}{s_{r_i}} \cup \bigcup_{\forall s_i \in S_o: s_i \longrightarrow s \vee s \longrightarrow s_i}{s_i}$ and
  $T_r^l = \bigcup_{\forall (s,t_{r_i}) \in R_s^l}{t_{r_i}} \cup \bigcup_{\forall t_i \in T_o: src(t'_i) = s \vee tar(t'_i) = s}{t'_i}$.
  
  We denote by $R_t^l(SC_o) = SC_r^l$ the local application of rule R2 on a transition $t \in T_o$, where $SC_r^l$ consists of solely the newly created states and transitions, and their immediate neighbors, \ie
  $S_r^l = \bigcup_{\forall (t,s_{r_i}) \in R_s^l}{s_{r_i}} \cup \{src(t), tar(t)\}$ and
  $T_r^l = \bigcup_{\forall (t,t_{r_i}) \in R_s^l}{t_{r_i}}$.
  
  The application of the five other rules can be reduced to the local refinements corresponding to R1 and R2.
\end{defn}

\begin{lemma}[Soundness: Local Rule is a Refinement]\label{lem:sound}
  Each refinement rule R1 through R7 creates local refinements restricted to the elements of the statechart being refined and satisfy the four refinement conditions, \ie $R^l \in \Re$.
\end{lemma}
\begin{proof}
  %It suffices to prove that R1 and R2 are valid refinements because the notion of refinement is naturally extended to the other Statecharts constructs that can be reduced to states and transitions through flattening.
  For R1, let $R_{s_o}^l(SC_o) = SC_r$ and $ST_r \subseteq S_r \cup T_r$ be the set of states and transitions $s_o$ is refined into.
  Then $\forall st_{r_i} \in ST_r, (s_o, st_{r_i}) \in R_{t_o}^l$ and condition (1) holds.
  %If $s_o$ is refined into a basic state $s_r \in S_r$, then $(s_o,s_r) \in R_{s_o}^l$.
  %Otherwise, $s_o$ is refined into an AND- or OR-state, then $(s_o,s_{r_1}),\ldots,$ $(s_o,s_{r_n}),(s_o,t_{r_1}),\ldots,(s_o,t_{r_m}) \in R_{s_o}^l$ where $s_{r_1},\ldots,s_{r_n} \in S_r$ and $t_{r_1},\ldots,t_{r_m} \in T_r$ are all the newly created states and any transitions between them.
  %Therefore condition (1) is satisfied.
  Condition~(\ref{eq:ev-var-incl}) is satisfied by design since new variables can be introduced in the entry/exit actions of the new states and new events can be introduced on the new transitions.
  Condition~(\ref{eq:guard-incl}) does not apply.
  Condition~(\ref{eq:struct-incl}) does not apply in case $s_r$ is a basic state.
  Otherwise, consider the case where $s_o$ is the target of a transition $t_o$ originating from a state $s_o'$ in the original statechart, that is $t_o = (s_o',e,\epsilon,s_o)$, where $e \in E_o$, and $\epsilon \subseteq E_o$ is the set of output events of $t_o$.
  Then there is always a path from any $s_r'$ to $s_{r_i}$ in $S_r$, \ie $\forall s_{r_i} \exists t_{r_i} = (s_r',e,\epsilon,s_{r_i}) \in T_r$.
  Similarly, suppose $t_o = (s_o,e,\epsilon,s_o')$.
  Then $\forall s_{r_i} \exists t_{r_i} = (s_{r_i},e,\epsilon,s_r') \in T_r$.
  These are the result of flattening the composite state $s_r$.
  
  For R2, let $R_{t_o}^l(SC_o) = SC_r$ and $ST_r$ be the set of states and transitions $t_o = (s_o,e,\epsilon,s_o')$ is refined into.
  Then $\forall st_{r_i} \in ST_r, (t_o, st_{r_i}) \in R_{t_o}^l$ and condition (1) holds.
  Condition~(\ref{eq:ev-var-incl}) is satisfied by design as for R1.
  Condition~(\ref{eq:guard-incl}) is also satisfied by design per rule R2.2.
  Condition~(\ref{eq:struct-incl}) is also satisfied by design, because there is always a path from $s_r$ to $\{s_r'\}$ in the refined Statechart since rule R2.4 prevents dead paths and rule R2.3 satisfies the broadcast restriction in~(\ref{eq:struct-incl}).
  \qed
\end{proof}

\begin{proposition}[Refinement Relation Reflexivity]\label{prop:reflex}
  $\forall SC_o, (SC_o,id(SC_o)) \in \Re$.
\end{proposition}
\begin{proof}
  To demonstrate the reflexivity of $\Re$, we need to show that each refinement condition allows for the identity and consequently from Lemma 1, each refinement rule allows for the identity.
  For condition~(\ref{eq:inv-surj}), since the identity is a surjection, then $R^{-1}$ allows for the identity and therefore $R$ does because $id^{-1} = id$.
  Condition~(\ref{eq:ev-var-incl}) is satisfied since $\subseteq$ is reflexive.
  Condition~(\ref{eq:guard-incl}) is satisfied by setting $p = true$.
  Condition~(\ref{eq:struct-incl}) is satisfied since $s_r = s_o, s_r' = s_o'$ and $p_r = p_o$ in the second case.
  \qed
\end{proof}
%
It follows from proposition~\ref{prop:reflex} that the \emph{copy} operation of a statechart is a refinement: this is the identity refinement, denoted by $R_{id} \in \Re$.
The following defines that a rule application is a local refinement rule \emph{merged} with the identity refinement for all elements of the statechart untouched by the rule.
%
\begin{defn}[Rule Application]\label{def:refStep}
  The application of a refinement rule consists of the merge refinement of the identity $R_{id}$ and local refinement $R^l$, denoted $merge(R_{id}, R^l)$.
  Let $merge(R_{id}, R^l)(SC_o) = SC_r$ and $R_{id}(SC_o) = SC'$.
  Then the application of rule R1 is defined by $merge(R_{id}, R_s^l)(SC_o) = \langle S^l_r \cup S' \setminus \{s'\}, T^l_r \cup T', E^l_r \cup E', V^l_r \cup V', P^l_r \cup P', g^l_r \cup g' \setminus \bigcup_{\forall t'_i \in T': src(t'_i) = s' \vee tar(t'_i) = s'}{g(t'_i)}, en^l_r \cup en' \setminus \{en(s')\}, ex^l_r \cup ex' \setminus \{ex(s')\} \rangle$.
  
  Similarly, the application of rule R2 is defined by $merge(R_{id}, R_t^l)(SC_o) = \langle S^l_r \cup S', T^l_r \cup T' \setminus \{t'\}, E^l_r \cup E', V^l_r \cup V', P^l_r \cup P', g^l_r \cup g' \setminus \{g(t'_i)\}, en^l_r \cup en', ex^l_r \cup ex' \rangle$.
\end{defn}

The following shows that a rule application is a refinement by proving that the merge operation is a refinement.
%
\begin{lemma}[Rule Application is a Refinement]\label{lem:merge_refinement}\\
  Let $R = merge(R_{id}, R^l)$, then $\forall SC_o, (SC_o, R(SC_o)) \in \Re$.
\end{lemma}
\begin{proof}
  In what concerns condition~(\ref{eq:inv-surj}), we can always separate the merge of $R_{id}$ with a local refinement $R^l$ in three parts: $R_1 \subseteq R_{id}\setminus R^l$, $R_2 \subseteq R^l \setminus R_{id}$ and $R_3 \subseteq R_{id} \cap R^l$.
  $R_1 \cup R_3$ is is inversely surjective because it is a subset of $R_{id}$.
  From lemma~\ref{lem:sound}, we have that $R^l$ satisfies condition~(\ref{eq:inv-surj}).
  Furthermore, note that the domain of $R^{l^{-1}}$ has no common elements with the domain of $R_{id}^{-1}$.
  Therefore, since $R^{l^{-1}}$ is surjective, $R_1 \cup R_2 \cup R_3 = merge(R_{id},R^l)$ is inversely surjective.
  Conditions~(\ref{eq:ev-var-incl}) and~(\ref{eq:guard-incl}) are trivially satisfied by construction.
  Condition~(\ref{eq:struct-incl}) holds because, from lemma~\ref{lem:sound}, both cases of local refinement rules R1 or R2 preserve structural inclusion by construction.
  A corollary of this proposition is that a rule application is a refinement.
  \qed
\end{proof}

\begin{proposition}[Refinement Relation Transitivity]\label{prop:refinement_trans}
  $\forall SC_o, SC_r = R_1(SC_o) \wedge SC_{r'} = R_2(SC_r) \Rightarrow \exists R_3 = R_1 \circ R_2: SC_{r'} = R_3(SC_o)$, for $ R_1,R_2,R_3 \in \Re$.
\end{proposition}
\begin{proof}
  To demonstrate the transitivity of $\Re$, we need to show that each refinement condition is transitive.
  Consequently, from Lemma 1, the composition of any two refinement rules still satisfies all four refinement conditions.
  $R_3^{-1} = R_2^{-1} \circ R_1^{-1}$ is a surjection, hence condition~(\ref{eq:inv-surj}) is satisfied.
  $\subseteq$ is a transitive relation, hence condition~(\ref{eq:ev-var-incl}) is satisfied.
  $g(t_r') = g(t_r) \wedge p' = g(t_o) \wedge p \wedge p'$, hence condition~(\ref{eq:guard-incl}) is satisfied.
  In what concerns condition~(\ref{eq:struct-incl}) we have that either (i) $s_r\stackrel{e[p_r]}{\longrightarrow}s_r''\stackrel{*}{\longrightarrow}s_r'''\stackrel{[p_r]/x}{\longrightarrow}s_r' \in LTS(SC_r)^{*}$ or (ii) $s_r\stackrel{e[p_r]/x}{\longrightarrow}s_r' \in LTS(SC_r)$.
  In case (i) we necessarily have that $s_{r'}\stackrel{e[p_{r'}]}{\longrightarrow}s_{r'}''\stackrel{*}{\longrightarrow}s_{r'}'''\stackrel{[p_r]/x}{\longrightarrow}s_{r'}'
  \in LTS(SC_{r'})^{*}$.
  In case (ii) we can have either $s_{r'}\stackrel{e[p_{r'}]}{\longrightarrow}s_{r'}''\stackrel{*}{\longrightarrow}s_{r'}'''\stackrel{[p_r]/x}{\longrightarrow}s_{r'}' \in LTS(SC_{r'})^{*}$ \mbox{~~or~~} $s_{r'}\stackrel{e[p_{r'}]/x}{\longrightarrow}s_{r'}' \in LTS(SC_{r'})$, hence condition~(\ref{eq:struct-incl}) is satisfied.
   \qed
\end{proof}

\begin{defn}[Sequence of Rule Applications]\label{def:refSeq}
  A sequence of rule applications is the composition of zero or more rule applications.
\end{defn}

\begin{proposition}[Sequence of Rule Applications is a Refinement]\\
  $\forall SC_o, SC_r = merge(R_{id}, R_1^l)(SC_o) \wedge SC_{r'} = merge(R_{id}, R_2^l)(SC_r)$ \\
  $\Rightarrow \exists merge(R_{id}, R_3^l) = merge(R_{id}, R_1^l) \circ merge(R_{id}, R_2^l):$ \\
  $SC_{r'} = merge(R_{id}, R_3^l)(SC_o)$, for $ R_1^l,R_2^l,R_3^l \in \Re$.
\end{proposition}
\begin{proof}
  The proof follows from lemma~\ref{lem:merge_refinement} and proposition~\ref{prop:refinement_trans}.
  \qed
\end{proof}

Therefore, conceptually, every rule application is a valid refinement and a sequence of rule applications is also a refinement.
% Consequently, the Statecharts refinement scheme we propose is also transitive:
% if $SC_2$ is a refinement of $SC_1$ and $SC_3$ is a refinement of a $SC_2$, then $SC_3$ is a refinement of $SC_1$.
This enables modelers to define multi-step refinements and therefore allows for incrementally refining Statecharts.
